Generating Content for HDR Deghosting from Frequency View

Recovering ghost-free High Dynamic Range (HDR) images from multiple Low Dynamic Range (LDR) images becomes challenging when the LDR images exhibit saturation and significant motion. Recent Diffusion Models (DMs) have been introduced in HDR imaging field, demonstrating promising performance, particularly in achieving visually perceptible results compared to previous DNN-based methods. However, DMs require extensive iterations with large models to estimate entire images, resulting in inefficiency that hinders their practical application. To address this challenge, we propose the Low-Frequency aware Diffusion (LF-Diff) model for ghost-free HDR imaging. The key idea of LF-Diff is implementing the DMs in a highly compacted latent space and integrating it into a regression-based model to enhance the details of reconstructed images. Specifically, as low-frequency information is closely related to human visual perception we propose to utilize DMs to create compact low-frequency priors for the reconstruction process. In addition, to take full advantage of the above low-frequency priors, the Dynamic HDR Reconstruction Network (DHRNet) is carried out in a regression-based manner to obtain final HDR images. Extensive experiments conducted on synthetic and real-world benchmark datasets demonstrate that our LF-Diff performs favorably against several state-of-the-art methods and is 10$\times$ faster than previous DM-based methods.

==> sec/0_abstract.tex <==
\begin{abstract}
Recovering ghost-free high dynamic range (HDR) images from multiple low dynamic range (LDR) images becomes challenging when the LDR images exhibit saturation and significant motion.
%
Recent diffusion models (DMs) have been introduced in HDR imaging, demonstrating promising performance, particularly in achieving visually perceptible results compared to previous DNN-based methods. 
%
However, 
% the standard DMs 
they require extensive iterations with large models to estimate entire images, resulting in inefficiency that hinders their practical application. 
% 
To address this challenge, we propose the Low-Frequency aware Diffusion (LF-Diff) model, including Low-frequency Prior Extraction Network (LPENet) and Dynamic HDR reconstruction Network (DHRNet) for ghost-free HDR imaging.
LF-Diff model avoids generating the contents from full-resolution features and improves the efficiency of the whole framework.
% has the powerful generation ability for saturated regions.
%
% Specifically, we 
To generate low-frequency priors for image reconstruction, the key idea of LPENet is to implement the DMs in a highly compacted latent space, which has the powerful generation ability for saturated regions.
%
In addition, to take full advantage of the low-frequency priors, the Dynamic HDR reconstruction Network (DHRNet) is carried out using a regression-based framework to obtain final HDR images, consisting of Prior Integration Module (PIM) and Feature Refinement Module (FRM).
% ensuring the efficiency of the DMs within the highly compact latent space. 
% 
Concretely, PIM efficiently integrates the low-frequency priors into the regression-based model to generate the contents of the unobserved regions, while FRM explicitly separates high and low-frequency features and processes them individually using distinct mechanisms tailored to their respective frequencies. 
%
Comprehensive experiments conducted on synthetic and real-world benchmark datasets demonstrate that our LF-Diff outperforms state-of-the-art methods.
% % Recovering ghost-free High Dynamic Range (HDR) images from multiple Low Dynamic Range (LDR) images becomes challenging when the LDR images exhibit saturation and significant motion. 
% Recovering ghost-free HDR images from multiple LDR images becomes challenging when the LDR images exhibit saturation and significant motion. 
% % Recent diffusion models show realistic and detailed image generation and motivate us to introduce them to HDR imaging for recovering human-eye perceptible results.
% Recent diffusion models have demonstrated realistic and detailed image generation, inspiring us to incorporate them into HDR imaging processes to achieve results that are visually pleasing and natural to the human eye.
% % Recent Diffusion models (DMs) have been introduced in HDR imaging and have shown promising performance, especially in achieving human-eye perceptible results. 
% However, unlike image synthesis methods that generate each pixel from scratch, LDR images already provides most of the necessary information. 
% Traditional DMs, which involve extensive iterations on large models to estimate entire images or feature maps, are inefficient. 
% % Thus, traditional DMs running massive iterations on a large model to estimate whole images or feature maps is inefficient. 
% To address this issue, we propose the Low Frequency Aware Diffusion Model (LF-Diff), for ghost-free HDR imaging.


% Comprehensive experiments on synthetic and real-world benchmark datasets demonstrate that our LF-Diff outperforms state-of-the-art methods.
\end{abstract}

% \begin{abstract}
% Recovering ghost-free high dynamic range (HDR) images from multiple low dynamic range (LDR) images becomes challenging when the LDR images exhibit saturation and significant motion. Recent diffusion models (DMs) have been introduced in HDR imaging, demonstrating promising performance, particularly in achieving visually perceptible results compared to previous DNN-based methods. However, DMs require extensive iterations with large models to estimate entire images, resulting in inefficiency that hinders their practical application. To address this challenge, we propose the Low-Frequency aware Diffusion (LF-Diff) model for ghost-free HDR imaging. The key idea of LF-Diff is implementing the DM in a highly compacted latent space and integrating it into a regression-based model to enhance the details of reconstructed images. Specifically，as low-frequency information is closely related to human visual perception we propose to utilize DMs to create compact low-frequency priors for the reconstruct process. In addition, to take full advantage of above low-frequency priors, the Dynamic HDR reconstruction Network (DHRNet) is carried out in a regression-based manner to obtain final HDR images, consisting of Prior Integration Module (PIM) and Feature Refinement Module (FRM). While PIM efficiently fuses the LPR with intermediate features of DHRNet, FRM further processes the fused features to reconstruct high-quality HDR images. Meanwhile, the highly compact latent
% space ensures the efficiency of the DM. Comprehensive experiments conducted on synthetic and real-world benchmark datasets demonstrate that our LF-Diff outperforms state-of-the-art methods.
% \end{abstract}
